Learning MPC for Interaction-Aware Autonomous Driving: A Game-Theoretic Approach

We consider the problem of interaction-aware motion planning for automated vehicles in general traffic situations. We model the interaction between the controlled vehicle and surrounding road users using a generalized potential game, in which each road user is assumed to minimize a common cost function subject to shared (collision avoidance) constraints. We propose a quadratic penalty method to deal with the shared constraints and solve the resulting optimal control problem online using an Augmented Lagrangian method based on PANOC. Secondly, we present a simple methodology for learning preferences and constraints of other road users online, based on observed behavior. Through extensive simulations in a highway merging scenario, we demonstrate the practical efficacy of the overall approach as well as the benefits of the proposed online learning scheme.

==> images/carDrawing.tex <==
\definecolor{roadborder}{HTML}{97adc6}
\definecolor{road}{HTML}{65758e}
\definecolor{stripes}{rgb}{1,1,1}
\definecolor{grass}{HTML}{bced9c}
\definecolor{windshield}{HTML}{cfe3f9}
\definecolor{car1color}{HTML}{267de0}
\definecolor{car2color}{HTML}{e04825}
\definecolor{car3color}{HTML}{FF4422}

% ========================================
% DEFINE ROAD SEGMENTS AND CARS
% ========================================
\tikzset{
	% pics/road/.style n args={4}{code={
	% 	\def\roadW{#1}
	% 	\def\roadL{#2}
	% 	\def\lineL{2}
	% 	\pgfmathsetmacro\nLines{int(floor(\roadL/\lineL))}
	% 	% \def\nLines{}
	% 	\fill[fill=road] (0,{-0.5*\roadW}) rectangle ({\roadL}, {0.5*\roadW}); 
	% 	\foreach \i in {0,...,{\nLines}}
	% 	{	
	% 		\fill[fill=stripes] ({\i*\lineL}, {-0.01*\roadW}) rectangle ({(\i+0.8)*\lineL}, {0.01*\roadW});
	% 	}
		% 
	% 	\fill[fill=roadborder] (0, {0.5*\roadW}) rectangle ({\roadL}, {0.5*\roadW+2}); 
	% 	\fill[fill=roadborder] (0, {-0.5*\roadW}) rectangle ({\roadL}, {-0.5*\roadW-2});
% 
	% 	\ifthenelse {\isempty{#4}}{}
	% 			{\fill[fill=stripes] (0.0*\roadW,{0.0*\roadW}) rectangle ({0.05*\roadW}, {0.45*\roadW});
	% 			}						
	% }},
	pics/car/.style args={#1}{
		code={
			\def\carw{3}
			\def\carh{6.5}
			% 
			% \draw [help lines, #1!10] (0,0) grid (\carw, \carh);
			\fill[fill=#1, rounded corners=20] (\carw,0) -- ++(0, \carh) -- ++(-\carw, 0) [rounded corners=30] -- ++(0, -\carh) -- cycle;
			% 
			%--------------------
			% Front windshield 
			%--------------------
			\def\winmarginy{2}
			\def\winh{1}
			
			\def\centerY{7}
			\def\rad{\centerY-\winmarginy}
			\def\theta{15} 
			\def\xtop{0.5*(\carw) + (\rad)*sin(\theta)}
			\def\ytop{\centerY - (\rad)*cos(\theta)}
			
			\def\xbot{0.5*(\carw) - (\rad-\winh)*sin(\theta)}
			\def\ybot{\centerY - (\rad-\winh)*cos(\theta)}
			
			\def\startalpha{270+\theta}
			\def\endalpha{270-\theta}
			
			\fill[fill=windshield, ] ({\xtop}, {\ytop}) arc({\startalpha}:{\endalpha}:{\rad}) -- ({\xbot}, {\ybot}) arc({\endalpha}:{\startalpha}:{\rad-\winh});
			
			%--------------------
			% Back windshield 
			%--------------------
			\def\winmarginy{0.7}
			\def\winh{0.5}
			
			\def\centerY{\carw-8}
			\def\theta{18}
			\def\rad{\carw+\centerY-\winmarginy}
			\def\xtop{0.5*(\carw) + (\rad)*sin(\theta)}
			\def\ytopback{\carw- (\centerY - (\rad)*cos(\theta))}
			
			\def\xbot{0.5*(\carw) - (\rad-\winh)*sin(\theta)}
			\def\ybot{\carw- (\centerY - (\rad-\winh)*cos(\theta))}
			
			\def\startalpha{270+\theta}
			\def\endalpha{270-\theta}
			
			\fill[fill=windshield] ({\xtop}, {\ytopback}) arc({\startalpha}:{\endalpha}:{\rad}) -- ({\xbot}, {\ybot}) arc({\endalpha}:{\startalpha}:{\rad-\winh});
			
			%--------------------
			% left window 
			%--------------------
			
			\def\centerleft{-4}
			\def\marginx{0.2}
			\def\radius{\marginx-\centerleft}
			\def\angle{20}
			\def\top{0.5*\carh + (\radius)*sin(\angle)}
			\def\bottom{0.5*\carh - (\radius)*sin(\angle)}
			
			\fill[fill=windshield, ] ({\marginx}, {\top}) arc(0.5*\angle: -0.5*\angle: {\radius}) -- cycle;
			\fill[fill=windshield, ] ({\carw-\marginx}, {\top}) arc(180-0.5*\angle: 180+0.5*\angle: {\radius}) -- cycle;
										arc({\endalpha}:{\startalpha}:{\rad-\winh});
			
			% ----------------------------
			% Left mirror 
			% ----------------------------
			\def\mirrorY{0.4*\carh}
			\fill[fill=#1] ({0.05*\carw}, {\mirrorY}) arc(0:-180:0.3) -- cycle;
			\fill[fill=#1] ({0.95*\carw}, {\mirrorY}) arc(-180:0:0.3) -- cycle;
			% \node[text=windshield, anchor=east] at ({0.5*\carw}, {0.5*\carh}) {\textbf{#2}};
		}
	}
}

% \tikzset{
% 	% pics/road/.style n args={4}{code={
% 	% 	\def\roadW{#1}
% 	% 	\def\roadL{#2}
% 	% 	% \def\lineL{2}
% 	% 	% \pgfmathsetmacro\nLines{int(floor(\roadL/\lineL))}
% 	% 	% % \def\nLines{}
% 	% 	% \fill[fill=road] (0,{-0.5*\roadW}) rectangle ({\roadL}, {0.5*\roadW}); 
% 	% 	% \foreach \i in {0,...,{\nLines}}
% 	% 	% {	
% 	% 	% 	\fill[fill=stripes] ({\i*\lineL}, {-0.01*\roadW}) rectangle ({(\i+0.8)*\lineL}, {0.01*\roadW});
% 	% 	% }
% 	% 	%
% 	% 	% \fill[fill=roadborder] (0, {0.5*\roadW}) rectangle ({\roadL}, {0.5*\roadW+2}); 
% 	% 	% \fill[fill=roadborder] (0, {-0.5*\roadW}) rectangle ({\roadL}, {-0.5*\roadW-2});
% 	% 	%
% 	% 	% \ifthenelse {\isempty{#4}}{}
% 	% 	% 		{\fill[fill=stripes] (0.0*\roadW,{0.0*\roadW}) rectangle ({0.05*\roadW}, {0.45*\roadW});
% 	% 	% 		}						
% 	% }},
% 	pics/car/.style n args={1}{
% 	code={
% 	% \def\carw{3}
% 	% \def\carh{6.5}
% 	% \def\winmarginx{0.2}
% 	% \def\wintiltinward{0.2}
% 	% \def\winradiusfront{7}
% 	% \def\winradiusback{10}
% 	% \def\winmarginy{2}
% 	% \def\winh{1}
% 	% \def\alphafront{30}
% 	% \def\alphaback{120}
% 	% 
% 	% % \draw [help lines, #1!10] (0,0) grid (\carw, \carh);
% 	% \fill[fill=#1, rounded corners=20] (\carw,0) -- ++(0, \carh) -- ++(-\carw, 0) [rounded corners=30] -- ++(0, -\carh) -- cycle;
% % 
% 	% %--------------------
% 	% % Front windshield 
% 	% %--------------------
% 	% 	\def\centerY{7}
% 	% 	\def\rad{\centerY-\winmarginy}
% 	% 	\def\theta{15} 
% 	% 	\def\xtop{0.5*(\carw) + (\rad)*sin(\theta)}
% 	% 	\def\ytop{\centerY - (\rad)*cos(\theta)}
% % 
% 	% 	\def\xbot{0.5*(\carw) - (\rad-\winh)*sin(\theta)}
% 	% 	\def\ybot{\centerY - (\rad-\winh)*cos(\theta)}
% % 
% 	% \def\startalpha{270+\theta}
% 	% \def\endalpha{270-\theta}
% % 
% 	% 	\fill[fill=windshield, ] ({\xtop}, {\ytop}) arc({\startalpha}:{\endalpha}:{\rad}) -- ({\xbot}, {\ybot}) arc({\endalpha}:{\startalpha}:{\rad-\winh});
% 	% 
% 	% %--------------------
% 	% % Back windshield 
% 	% %--------------------
% % 
% 	% \def\winmarginy{0.7}
% 	% \def\centerY{\carw-8}
% 	% \def\winh{0.5}
% 	% \def\theta{18} 
% 	% 	\def\rad{\carw+\centerY-\winmarginy}
% 	% \def\xtop{0.5*(\carw) + (\rad)*sin(\theta)}
% 	% 	\def\ytopback{\carw- (\centerY - (\rad)*cos(\theta))}
% % 
% 	% 	\def\xbot{0.5*(\carw) - (\rad-\winh)*sin(\theta)}
% 	% 	\def\ybot{\carw- (\centerY - (\rad-\winh)*cos(\theta))}
% % 
% 	% \def\startalpha{270+\theta}
% 	% \def\endalpha{270-\theta}
% % 
% 	% 	\fill[fill=windshield] ({\xtop}, {\ytopback}) arc({\startalpha}:{\endalpha}:{\rad}) -- ({\xbot}, {\ybot}) arc({\endalpha}:{\startalpha}:{\rad-\winh});
% % 
% 	% %--------------------
% 	% % left window 
% 	% %--------------------
% 	% 
% 	% \def\centerleft{-4}
% 	% \def\marginx{0.2}
% 	% \def\radius{\marginx-\centerleft}
% 	% \def\angle{20}
% 	% \def\top{0.5*\carh + (\radius)*sin(\angle)}
% 	% \def\bottom{0.5*\carh - (\radius)*sin(\angle)}
% 	% 
% 	% \fill[fill=windshield, ] ({\marginx}, {\top}) arc(0.5*\angle: -0.5*\angle: {\radius}) -- cycle;
% 	% 	\fill[fill=windshield, ] ({\carw-\marginx}, {\top}) arc(180-0.5*\angle: 180+0.5*\angle: {\radius}) -- cycle;
% 	% 	arc({\endalpha}:{\startalpha}:{\rad-\winh});
% %
% 	% 	% ----------------------------
% 	% 	% Left mirror 
% 	% 	% ----------------------------
% 	% 	\def\mirrorY{0.4*\carh}
% 	% 	\fill[fill=#1] ({0.05*\carw}, {\mirrorY}) arc(0:-180:0.3) -- cycle;
% 	% 	\fill[fill=#1] ({0.95*\carw}, {\mirrorY}) arc(-180:0:0.3) -- cycle;
% 	}
% 	}
% }


==> images/traffikz.tex <==
        % ========================================
        % DEFINE COLORS 
        % ========================================

        \definecolor{roadborder}{HTML}{97adc6}
        \definecolor{road}{HTML}{65758e}
        \definecolor{stripes}{rgb}{1,1,1}
        \definecolor{grass}{HTML}{bced9c}
        \definecolor{windshield}{HTML}{cfe3f9}
        \definecolor{car1color}{HTML}{267de0}
        \definecolor{car2color}{HTML}{e04825}
        \definecolor{car3color}{HTML}{FF4422}

        % ========================================
        % DEFINE ROAD SEGMENTS AND CARS
        % ========================================
        \tikzset{
            pics/pedestrian/.style args={#1}{code={
                \def\shoulderwidth{2}
                \def\thickness{0.5}
                \fill[fill=#1, rounded corners] ({-0.5*\thickness}, {-0.5*\shoulderwidth}) rectangle ({0.5*\thickness}, {0.5*\shoulderwidth});
                \draw[fill=black, draw=none] (0,0) circle ({0.2*\shoulderwidth});
            }},
            pics/bicycle/.style args={#1}{code={
                \def\bikelength{4.5}
                \def\bikewidth{0.3}
                \fill[fill=black!80, rounded corners] (0, {-0.5*\bikewidth}) rectangle ({0.3*\bikelength}, {0.5*\bikewidth});
                \fill[fill=black!80, rounded corners] ({0.5*\bikelength}, {-0.5*\bikewidth}) rectangle ({\bikelength}, {0.5*\bikewidth});
                \fill[fill=black!70, rounded corners] ({0.5*\bikelength}, {-\bikewidth}) rectangle ({0.85*\bikelength}, {\bikewidth});

                % \fill[fill=#1, rounded corners] (0, {-0.5*\bikewidth}) rectangle ({\bikelength}, {0.5*\bikewidth});
                % \fill[rounded corners]
                \fill[fill=black!10, rounded corners] ({0.27*\bikelength}, {3*\bikewidth}) rectangle ({0.31*\bikelength}, {-3*\bikewidth});
                \fill[fill=black!10, rounded corners] ({0.27*\bikelength}, {3*\bikewidth}) rectangle ({0.31*\bikelength}, {-3*\bikewidth});

                \fill[fill=#1] ({0.43*\bikelength}, {3.3*\bikewidth}) arc (90:-90:{3.3*\bikewidth});
                \draw[fill=black, line width=0.35cm, rounded corners] ({0.44*\bikelength}, {2.6*\bikewidth}) -- ({0.27*\bikelength}, {3*\bikewidth});
                \draw[fill=black, line width=0.35cm, rounded corners] ({0.44*\bikelength}, {-2.6*\bikewidth}) -- ({0.27*\bikelength}, {-3*\bikewidth});

                \draw[fill=black, draw=none] ({0.4*\bikelength},0) circle ({0.1*\bikelength});
            }},
            pics/road/.style n args={4}{code={
                \def\roadW{#1}
                \def\roadL{#2}
                \def\lineL{2}
                \pgfmathsetmacro\nLines{int(floor(\roadL/\lineL))}
                % \def\nLines{}
                \fill[fill=road] (0,{-0.5*\roadW}) rectangle ({\roadL}, {0.5*\roadW}); 
                \foreach \i in {0,...,{\nLines}}
                {   
                    \fill[fill=stripes] ({\i*\lineL}, {-0.01*\roadW}) rectangle ({(\i+0.8)*\lineL}, {0.01*\roadW});
                }
                
                \fill[fill=roadborder] (0, {0.5*\roadW}) rectangle ({\roadL}, {0.5*\roadW+2}); 
                \fill[fill=roadborder] (0, {-0.5*\roadW}) rectangle ({\roadL}, {-0.5*\roadW-2});

                \ifthenelse {\isempty{#4}}{}
                        {\fill[fill=stripes] (0.0*\roadW,{0.0*\roadW}) rectangle ({0.05*\roadW}, {0.45*\roadW});
                        }                       
            }},
            pics/car/.style args={#1}{
            code={
            \def\carw{3}
            \def\carh{6.5}
            \def\winmarginx{0.2}
            \def\wintiltinward{0.2}
            \def\winradiusfront{7}
            \def\winradiusback{10}
            \def\winmarginy{2}
            \def\winh{1}
            \def\alphafront{30}
            \def\alphaback{120}
            
            % \draw [help lines, #1!10] (0,0) grid (\carw, \carh);
            \fill[fill=#1, rounded corners=20] (\carw,0) -- ++(0, \carh) -- ++(-\carw, 0) [rounded corners=30] -- ++(0, -\carh) -- cycle;

            %--------------------
            % Front windshield 
            %--------------------
            \def\centerY{7}
            \def\rad{\centerY-\winmarginy}
            \def\theta{15} 
            \def\xtop{0.5*(\carw) + (\rad)*sin(\theta)}
            \def\ytop{\centerY - (\rad)*cos(\theta)}

            \def\xbot{0.5*(\carw) - (\rad-\winh)*sin(\theta)}
            \def\ybot{\centerY - (\rad-\winh)*cos(\theta)}

            \def\startalpha{270+\theta}
            \def\endalpha{270-\theta}

            \fill[fill=windshield, ] ({\xtop}, {\ytop}) arc({\startalpha}:{\endalpha}:{\rad}) -- ({\xbot}, {\ybot}) arc({\endalpha}:{\startalpha}:{\rad-\winh});
            
            %--------------------
            % Back windshield 
            %--------------------

            \def\winmarginy{0.7}
            \def\centerY{\carw-8}
            \def\winh{0.5}
            \def\theta{18} 
            \def\rad{\carw+\centerY-\winmarginy}
            \def\xtop{0.5*(\carw) + (\rad)*sin(\theta)}
            \def\ytopback{\carw- (\centerY - (\rad)*cos(\theta))}

            \def\xbot{0.5*(\carw) - (\rad-\winh)*sin(\theta)}
            \def\ybot{\carw- (\centerY - (\rad-\winh)*cos(\theta))}

            \def\startalpha{270+\theta}
            \def\endalpha{270-\theta}

            \fill[fill=windshield] ({\xtop}, {\ytopback}) arc({\startalpha}:{\endalpha}:{\rad}) -- ({\xbot}, {\ybot}) arc({\endalpha}:{\startalpha}:{\rad-\winh});

            %--------------------
            % left window 
            %--------------------

            \def\centerleft{-4}
            \def\marginx{0.2}
            \def\radius{\marginx-\centerleft}
            \def\angle{20}
            \def\top{0.5*\carh + (\radius)*sin(\angle)}
            \def\bottom{0.5*\carh - (\radius)*sin(\angle)}

            \fill[fill=windshield, ] ({\marginx}, {\top}) arc(0.5*\angle: -0.5*\angle: {\radius}) -- cycle;
            \fill[fill=windshield, ] ({\carw-\marginx}, {\top}) arc(180-0.5*\angle: 180+0.5*\angle: {\radius}) -- cycle;
            arc({\endalpha}:{\startalpha}:{\rad-\winh});

            % ----------------------------
            % Left mirror 
            % ----------------------------
            \def\mirrorY{0.4*\carh}
            \fill[fill=#1] ({0.05*\carw}, {\mirrorY}) arc(0:-180:0.3) -- cycle;
            \fill[fill=#1] ({0.95*\carw}, {\mirrorY}) arc(-180:0:0.3) -- cycle;
            }
            }
        }
